Explaining Differences in Classes of Discrete Sequences

While there are many machine learning methods to classify and cluster sequences, they fail to explain what are the differences in groups of sequences that make them distinguishable. Although in some cases having a black box model is sufficient, there is a need for increased explainability in research areas focused on human behaviors. For example, psychologists are less interested in having a model that predicts human behavior with high accuracy and more concerned with identifying differences between actions that lead to divergent human behavior. This paper presents techniques for understanding differences between classes of discrete sequences. Approaches introduced in this paper can be utilized to interpret black box machine learning models on sequences. The first approach compares k-gram representations of sequences using the silhouette score. The second method characterizes differences by analyzing the distance matrix of subsequences. As a case study, we trained black box supervised learning methods to classify sequences of GitHub teams and then utilized our sequence analysis techniques to measure and characterize differences between event sequences of teams with bots and teams without bots. In our second case study, we classified Minecraft event sequences to infer their high-level actions and analyzed differences between low-level event sequences of actions.

==> removed_text.tex <==
% \subsubsection{Team Productivity}
% Prior studies have measured the amount of work performed by GitHub teams by counting the number of push events~\cite{muric2019collaboration}. 
% This approach works for repositories that have the \textit{shared repository} development model in which team members are granted push access.
% However, many large open-source repositories have the \textit{fork and pull} model in which all GitHub users are allowed to fork the repository, make changes and send a pull request to submit their contributions.
% To account for these repositories, in addition to push events, we included the number of accepted pull requests in the work of the team.
% Moreover, we believe that the communications between team members about code development are an important component of teamwork. Therefore, we included these types of comments in the tally of work. 
% Thus in order to measure the total work of a team, we tabulated a subset of the GitHub events for the team repository: push, issue comment, pull request review comment, and accepted pull request.

% For each team, we then calculated work per human (i.e. total work divided by the team size) to measure the productivity of the team.  For this analysis, we removed the events associated with the bot accounts.  Teams were then grouped according to size.
% We considered teams as small if they had two or three members, medium if they had between four and six contributors, and large if they had seven or more members. 
% Figure \ref{fig:productivity} illustrates differences between productivity of human-bot teams versus human teams. Human-bot teams are more productive regardless of their team sizes. 
% A t-test shows that the \textit{p-value} is less than $10^{-2}$ for team productivity in Figure~\ref{fig:productivity}. Therefore, as measured by the generation of GitHub events, the productivity of human-bot teams is significantly higher than the productivity of human teams.  This indicates that the bots are affecting the work process by modifying the type of events executed by human team members rather than reducing their overall quantity. 

% \begin{figure}[h!]
% \centerline{\includegraphics[width=0.9\linewidth]{figs/productivity.png}}
% \caption{Human-bot teams are more productive than human only ones, as measured by generation of work events.}
% \label{fig:productivity}
% \end{figure}





% To make sure that the observed differences are due to teamwork differences rather than the additional bot event activity,
% we also measured the silhouette score after removing bot activity  from human-bot team sequences. We still observed positive, although slightly lower, silhouette scores between team sequences.  This shows that using bots in GitHub teams not only affects the sequences of the teams but also changes the activities of the human members of the teams.






% Distance matrices for a randomly selected sequence are visualized in Figure~\ref{fig:distance_matrix} for different values of window sizes.
% For every subsequence, the distance matrix shows the position of all similar subsequences.
% In the heat-map plots of Figure~\ref{fig:distance_matrix} similarity is represented by redness.
% So for every row of the distance matrix, red blocks demonstrate repeats of similar subsequences.
% For smaller window sizes, blocks are smaller but the similarity is higher. 
% For a window size of 20, there are subsequences that perfectly match (zero distance).

% \begin{figure*}[h]
% \includegraphics[width=\textwidth]{figs/dm_scaled.png}
% \caption{Distance matrix of a randomly selected sequence for different values of window size. For every subsequence, the distance matrix shows the position of all similar subsequences.
% Similarity is represented by redness; red blocks demonstrate repeats of similar subsequences.  For smaller window sizes, the blocks are smaller but the similarity is higher.  Note that heat maps are scaled to lie between 0 to 100 to make comparison easier. }
% \label{fig:distance_matrix}
% \end{figure*}

% From distance matrices of sequences in our dataset, we created their matrix profiles.
% Figure \ref{fig:matrix_profiles} shows the corresponding matrix profile of the sequence in Figure \ref{fig:distance_matrix} for different window sizes.

% The trend of the matrix profile is independent of the window size, i.e. minimums and maximums occur at the same positions for different window sizes.
% Minimums of the matrix profile represent motifs of the sequence and maximums are related to discord or anomalies.
% Increasing the window sizes enlarges the distance between the most similar subsequences (e.g. distance between most similar subsequences is 40 for the window size of 100).
% For our remaining experiments, we choose $w=20$ as it finds more similar subsequences.

% \begin{figure*}[h]
% \includegraphics[width=\textwidth]{figs/mp.png}
% \caption{Matrix profile of the sequence in Figure \ref{fig:distance_matrix}. The trend of the matrix profile is independent of the window size.  Increasing the window sizes enlarges the distance between the most similar subsequences. }
% \label{fig:matrix_profiles}
% \end{figure*}




% Introduction to Human-bot teaming
%In 1960, JCR Licklider envisioned collaboration of humans and computers in his famous paper called "Man-Computer Symbiosis" \cite{licklider1960man}. Licklider anticipated that in this symbiotic partnership, humans will be involved in the complex tasks such as goal setting and hypothesizing while the computing machines will perform the routine tasks. He predicted that this symbiotic partnership is more effective in performing intellectual operations than human alone.
%Licklider's vision has definitely come true in the 21st century with technological advances in Artificial Intelligence.
%One of the areas that we can witness the collaboration of humans and machines is bots that are software development teammates in social coding platforms.


% Many machine learning methods lack explainability, in that, it is hard or impossible to understand why they classified or clustered a group of instances differently from another group.
% Although it seems challenging to interpret all types of data, in this study, we focused on one specific data type: discrete sequences.



%%%%%%%%%%%%%% SUMMARY %%%%%%%%%%%%%%%%%%%

%Our first approach converts sequences to their k-gram representations and then computes Term Frequency-Inverse Sequence Frequency or \textit{TF-ISF} vectors of sequences based on their k-gram. \textit{TF-ISF} is analogous to the \textit{TF-IDF} concept in information retrieval which aims to reflect the importance of various words in a collection of textual documents.
%After vectorizing sequences using \textit{TF-ISF}, our approach uses the silhouette score to quantify differences between groups of sequences.
%Silhouette score is a measurement used for evaluating clustering results.

%Our second approach is based on a time series analysis algorithm called matrix profiling \cite{yeh2016matrix}. 
%In matrix profiles, subsequences of the time series are compared against themselves by computing the distance between each pair of subsequences. 
%We modified the matrix profile algorithm to make it compatible with sequences.  The output of the matrix profile is then used to detect whether characteristics of groups of sequences such as complexity and novelty are different across groups.
%In this study, the matrix profile was used to characterize differences in the automation usage of teams. However, a matrix profile is a powerful tool that makes many data mining tasks simple and effortless. For example, motifs and discords can be detected using matrix profile \cite{torkamani2017survey,yeh2018time}. Moreover, using the matrix profile facilitates the classification and segmentation of sequences \cite{yeh2017matrix,yeh2018time,yeh2016matrix}.


%The contributions of this paper are as follows:
%    1) Provided two approaches for explaining differences between groups of discrete sequences;
%    2) Introduced a new matrix profile construction approach for discrete sequences.


% In many cases, sequences cannot directly be used as the input of machine learning models.
% However, machine learning methods can be applied to sequences converted to equal-length real-valued vectors.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% GitHub Apps, which are official GitHub bots, can automate developer tasks and potentially improve efficiency.  These bots are semi-autonomous and capable of executing a variety of teamwork and taskwork functions.  
% We hypothesize that different team coordination choices will manifest themselves as variations in event sequence patterns.

%% cmt
% We constructed three sequence classification models to predict whether the sequence was generated by a repository with bot support.  Our first classification model is a Support Vector Machine (SVM) that takes the vectorized k-gram representation of the sequences as input. Our second model is a LSTM (Long Short Term Memory) model with a sequence embedding layer for vectorization of the input sequence. The third model is a combination of CNN (Convolutional Neural Networks) and LSTM models. These results were compared with a simple length-based logistic regression model.  All models were able to distinguish whether an event sequence was generated by a human only or human-bot team, with the neural network models achieving the best F1 score, 0.79, which was significantly better than the baseline. These results validate our hypothesis that the event sequences can be leveraged to detect teamwork differences.
% Analyzing event distributions alone was insufficient to reveal the subtle differences in human-bot vs.\ human only teamwork.  Hence we propose a new analytic approach to quantify the differences between two groups of sequences.
% First, we compared two groups of sequences by converting the sequences to k-gram representation vectors and measuring the silhouette score of the groups. Our results show that sequences of human teams are distinct from sequences of human-bot teams.
% Second, to understand differences between sequences, we created matrix profiles for all sequences and compared statistics and aggregated matrix profiles of the two groups.  Based on our analysis, human-bot teams have more novel event sequences. In contrast, human teams have more repetitive sequences, especially at the early stages of their work.




% cmt
% GitHub has an open API to collect metadata about users, repositories, and the activities of users on repositories. It also supports passive social media style interactions such as following repositories or developers. These features make it a powerful tool for analyzing the behavior of individual software engineers, development teams, and open source communities.

%Developers make changes to the code repository by pushing their content, while GitHub tracks the version control process. Any GitHub user can contribute to a repository by sending a pull request. Repository maintainers review pull requests, discuss possible modifications in the comments, and decide whether to accept or reject the requests.

%% Software
%% cmt
% Individual software developer behaviors have been widely studied due to their critical role in the tech business. For instance, Bao et al. analyzed developer turnover in two companies \cite{bao2017will} and created a model to predict whether a developer will leave based on monthly reports. Many software developers work in teams that are geographically dispersed and work asynchronously. Vasilescu et al. \cite{vasilescu2015data} created a data set of GitHub programmers' attributes, including location and gender. This data can be used to study the effects of gender and tenure diversity on team productivity and turnover.  A question of interest to the software engineering industry is examining the effects of adding collaborators; whether it makes teams more productive or merely adds free-riders?~\cite{muric2019collaboration} In contrast, our research focuses on team cognitive processes rather than individual developer differences.




% This body of work examines differences between contributors, including their varying influence on each other \cite{Blincoe2016:popular}, and their level and length of participation \cite{saadat2018initializing,Joblin:devcoord, vasilescu2015gender, Onoue:devchar}.

% Rather than interviewing teams on how they utilize automated development tools, our aim is to create new techniques that enable us to study the performance and cognitive processes of GitHub teams from analyzing their event sequences.   Event distributions have been used in previous work to learn team ``archetypes''.  These archetypes formed the basis of an agent-based model capable of forecasting developer activity~\cite{saadat2018initializing}.  However, we were unable to identify differences between human-only and human-bot teams based solely on the event distributions; instead we use event sequences to gain insight about subtle differences in the temporal dynamics of GitHub teams.



 
 
 %% cmt
%  Figure \ref{fig:codecov} shows an example of a GitHub bot, Codecov. 
%  Codecov\footnote{https://codecov.io/} is an example of a code coverage tool that provides testing support. Code coverage is a measurement used to express the percentage of lines of code that were executed by an automated test suite. 
%   A program with high test coverage has had more of its source code executed during testing and thus has a lower chance of containing undetected software bugs compared to a program with low test coverage.
%  The Codecov bot can improve code review workflow and quality.
 
 
%% cmt 
%  In an effort to support the study of software bots, Storey and Zagalsky identified different classes of bots commonly used in software development: 1) coding support 2) code testing 3) development operations 4) user support 5) documentation~\cite{Storey2016:botsDisrupt}.   Coding support bots assist with coding workflow efficiency. Testing support bots allow developers to offload the repetitive task of evaluating code.  DevOp bots bridge knowledge and communication gaps in software teams. User support bots communicate with software users and provide answers to frequently asked questions.  Documentation bots aggregate information from multiple sources into code  documentation. In most cases, the bots perform taskwork rather than teamwork functions, although some research has begun to explore how bots can improve teamwork by reducing conflict between developers~\cite{Lebeuf2017:botsFriction}.  

 
%  \begin{figure}
% \centerline{\includegraphics[width=0.9\linewidth]{figs/codecov_bot.png}}
% \caption{Example output from the GitHub bot, Codecov (Image downloaded from https://docs.codecov.io/docs/pull-request-comments)}
% \label{fig:codecov}
% \end{figure}

%% cmt 
%  The hope is that automating repetition in the software development process helps the developers focus on more meaningful tasks.  However, Wessel et al.~\cite{wessel2018} note that 
%  their adoption in a project does not yield significant increases in developer productivity according to some standard measures.
% Bernardo et al. \cite{bernardo2018studying} also observed that adopting Continuous Integration (CI) bots, surprisingly, only improves the time to deliver merged pull requests (PRs) for half of the teams but their investigation shows that the increase of PR submissions after CI is the cause of slower PR delivery.








% Developers make changes to the repository by pushing their content. To be able to push to a repository, users should have push privilege. This push-based developmental model is mainly used for smaller teams.
% Large open-source projects use pull-based developmental model in which, any GitHub user can contribute to a repository by forking (i.e. copying) the repository, making modifications and submitting their contributions by sending a pull request to the original repository. Repository maintainers review pull requests, discuss possible modifications in the comments, and decide whether to accept or reject the requests.
% GitHub users can report bugs or request new features in the issues section of repositories and other users can comment on the issues to discuss best approaches to address the issue or coordinate on who will work on the issue and how.
% Users can star a repository to bookmark it or to show their interest in a repository. GitHub also  allow users to follow repositories of their interest to get the latest update about them.
% Users can follow each other on GitHub and get informed about activities of developers they like.





% In our research, we need to predict which group each sequence of repository events belongs to.
% Creating a predictive model requires discriminative features.
% The approaches discussed in Section \ref{ss:kgram} and \ref{ss:matrix_profile} reveal whether the two groups of sequences are different from each other. For a dataset, if we infer, from the above methods, that two groups are distinct, a model can be trained to predict the group from the sequences themselves.

%\subsubsection{Support Vector Machines}
%The first supervised learning model we tested is one of the classical machine learning approaches.
%To use classic machine learning algorithms, we need equal length real-valued vectors.
%One of the challenges of the sequence classification problem is that sequences can vary in length.
% We convert sequences to vectors using the vectorization methods discussed in \ref{sss:seq2vec}.
%We use a k-gram representation for vectorizing the sequences in the dataset (more discussion in \ref{sss:seq2vec}) before employing a support vector machine (SVM) model to construct a predictive model.
%Support Vector Machines (SVM) is a very powerful and versatile machine learning model that works well on complex but small or medium size datasets.
%We chose SVM for this problem because it is effective in high dimensional spaces, specially, when the number of features is higher than the number of samples.
%In the k-gram representation of event sequences, the number of features is equal to the number of possible k-grams which is $n^k$ where $n$ is the distinct number of events. 

%\subsubsection{Neural Networks}
%Our second approach for sequence classification is using deep neural network models.
%Deep learning models, unlike classic algorithms such as SVM, do not require direct vectorization. 
%These models can have an embedding layer that converts the sequences to real-valued vectors.
%We test two different neural network architectures in this research.
%In both architectures, we use a Long Short Term Memory (LSTM) layer to learn representation for sequences.
%LSTMs are a type of Recurrent Neural Network that have achieved success in learning dependencies in different kinds of sequences such as sequence of words (i.e. text) and sequence of real values (i.e. time series). LSTMs are used in many Natural Language Processing tasks such as machine translation \cite{sutskever2014sequence}. LSTMs are also popular in time series prediction problems \cite{fu2016using}.
%Research shows that LSTMs are capable of modeling complex and non-linear feature interactions \cite{ogunmolu2016nonlinear}.
% LSTMs are also used for text classification which is a type of sequence classification task \cite{}.

%In addition, we test 1-Dimensional Convolutional Neural Networks (1D CNNs) which excel at learning the spatial structure in input data. CNNs are also used in many sequence models such as sentence classification, and language translation \cite{kim2014convolutional, kalchbrenner2013recurrent}.

%\subsubsection{Baseline}
%Our baseline is a simple Logistic Regression model. This model considers length of the input sequence as the only feature for the classification task.
% Convolutional neural networks (CNNs) excel at learning the spatial structure in input data.
% We use a 1-dimensional CNN layer to enable our model to recognize invariant features for two groups.
% Spatial features can be learned as sequences by an LSTM layer.

% In order to train a model that predict which group a sequence belong to, we used Long Short-Term Memory (LSTM) model.

% sequence to sequence learning




% Cosine Similarity
% Because TF-ISF vectors are long and sparse (mostly zeros) vectors their euclidean distance would be close to zero most of the time.


%Euclidean distance is the most commonly used method for measuring the distance between vectors. 
%It would work well if we had equal length sequences; however, if the length of sequences varies, Euclidean distance is higher between sequences that have larger length differences.

% Two common similarity method for TF-IDFs: cosine, Jaccard
%Hence, we use cosine similarity to measure the distance between vectors of sequences to eliminate the impact of sequence length.
%Cosine similarity calculates similarity by measuring the cosine of the angle between two vectors.
%Cosine-based distance can be easily obtained by subtracting cosine similarity from one:
%\begin{equation} \label{eq:cos}
%    d(i,j)=1-\frac{v_i.v_j}{\left \| v_i \right \| \left \| v_j \right \|}
%\end{equation}
%where $d(i,j)$ is the distance between vector $v_i$ and $v_j$.

% Jaccard similarity is good for cases where duplication does not matter, 
% cosine similarity is good for cases where duplication matters while analyzing text similarity. 
% Since the frequency of k-grams matter to us, we used cosine similarity.




% The silhouette score (Equation \ref{eq:s}) is calculated using the mean intra-group distance ($a(i)$ in Equation \ref{eq:a}) and the mean nearest-group distance ($b(i)$ in Equation \ref{eq:b}) for each sequence $i$. 
% To find the distance between sequence $i$ and group $j$, the distances between $i$ and all sequences in group $j$ are found, and their average is calculated. 
% \begin{equation} \label{eq:a}
%     a(i)=\frac{1}{|G_i|-1}\sum_{j \in G_i, i \ne j} d(i, j)
% \end{equation}
% \begin{equation} \label{eq:b}
%     b(i)=\frac{1}{|G_i|}\sum_{j \in G_i} d(i, j)
% \end{equation}
% \begin{equation} \label{eq:s}
%     s(i)=\frac{b(i)-a(i)}{\max \left \{ a(i), b(i) \right\}}, \mbox{if } |G_i|>1
% \end{equation}
% and $s(i)=0, \mbox{if } |G_i|=1$.




%% MATRIX profile intro was here

% The main difference between matrix profiles on sequences versus time series is the distance calculation function. Euclidean distance is defined on real values and thus cannot be applied to sequences. Therefore, we use a distance function designed for discrete sequences: Hamming distance.


% % LCS
% Longest Common Subsequence (LCS) is a classic dynamic programming algorithm that finds the longest subsequence common between two sequences; $w-\mbox{len}(LCS)$ is the LCS-based distance metric between two subsequences of length $w$. 
% LCS time complexity is $O(w^2)$ where $w$ is the length of LCS input sequences. Hence the distance matrix calculation time complexity is $O(n^2w^2)$.









Figure \ref{fig:seq_len} shows the distribution of sequence lengths for human-bot teams and the downsampled group of human teams. Human only teams have shorter average sequence lengths; the variance of the sequence lengths is also smaller in human teams. 
% As demonstrated in Section \ref{ss:res_classification}, sequence length alone is not a predictor of the team type that generated that sequence.

% seq_len
\begin{figure}[h!]
\centerline{\includegraphics[width=0.7\linewidth]{figs/seq_len.png}}
\caption{Human-bot teams have longer sequences on average; however this is not a strong predictor of team type.}
\label{fig:seq_len}
\end{figure}
